Physics-Grounded Causal Auditing of End-to-End Driving Planners

End-to-end (E2E) autonomous-driving planners trained by imitation are prone to statistical shortcuts: they associate scene elements that merely co-occur with expert actions (a roadside object, a building facade) with driving decisions, rather than the variables that causally determine them. Such causal confusion silently compromises reliability in long-tail scenarios, and it is difficult to detect, because prevailing open-loop metrics (L2 displacement and collision rate) are dominated by ego status and do not indicate whether a planner depends on spurious cues. Existing remedies based on causal-intervention training require retraining large models and cannot audit a planner that is already deployed. We present CADET, a training-free framework that audits, benchmarks, and repairs spurious reliance in pretrained E2E planners without any parameter update.

==> figures/fig1/panel_a.tex <==
% =====================================================================
%  Fig. 1, panel (a): the frozen planner and the scene it emits.
%  Local frame: (0,0) bottom-left, 4.15 x 4.60 cm.
% =====================================================================
\begin{scope}[shift={(\pAx,\pRowy)}]
\def\W{4.15}\def\H{4.60}
\draw[panel] (0,0) rectangle (\W,\H);

% ---- heading --------------------------------------------------------
\node[ptitle] at (0.16,\H-0.30) {(a) Frozen E2E planner};
\node[psub] (asub) at (0.16,\H-0.55) {SparseDrive, weights frozen};
\pic at ([xshift=1.9mm]asub.east) {snow};

% ---- inference chain -------------------------------------------------
\node[card, inner xsep=2.4pt, inner ysep=2.2pt, font=\cdtiny,
      anchor=west] (cam) at (0.16,\H-0.97) {$6{\times}$ cams};
\node[card, inner xsep=2.4pt, inner ysep=2.2pt, font=\cdtiny,
      anchor=west] (per) at ([xshift=2.6mm]cam.east) {perception};
\node[card, inner xsep=2.4pt, inner ysep=2.2pt, font=\cdtiny,
      anchor=west] (pln) at ([xshift=2.6mm]per.east) {planning head};
\draw[flow] (cam) -- (per);
\draw[flow] (per) -- (pln);
\draw[flow] (pln.south) -- ++(0,-0.18);

% ---- scene well ------------------------------------------------------
\draw[well] (0.16,0.72) rectangle (\W-0.16,3.32);

% forward-looking corridor, ego at the bottom
\def\rb{0.92}\def\rt{3.14}
\fill[cdBlueF] (0.84,\rb) -- (3.31,\rb) -- (2.45,\rt) -- (1.70,\rt) -- cycle;
\draw[cdBlue!38, line width=0.4pt]
  (0.84,\rb) -- (1.70,\rt)  (3.31,\rb) -- (2.45,\rt);
\draw[cdBlue!30, line width=0.35pt, dash pattern=on 1.5pt off 1.5pt]
  (2.075,\rb) -- (2.075,\rt);
\node[note, anchor=north west, text=cdBlue!62!black] at (0.24,3.26)
  {drivable corridor};

% ego vehicle
\fill[cdInk!88, rounded corners=0.7pt] (1.80,1.06) rectangle (2.35,1.38);
\node[note, anchor=east, text=cdSlate] at (0.86,1.22) {ego};

% planned waypoints
\foreach \y in {1.50,1.68,1.86,2.04}{\fill[cdBlue] (2.075,\y) circle (0.038);}
\node[note, anchor=east, text=cdBlue!80!black] at (1.96,1.77) {plan $a$};

% in-corridor lead vehicle
\draw[fill=cdGreenF, draw=cdGreen, line width=0.55pt, rounded corners=0.7pt]
  (1.865,2.40) rectangle (2.285,2.62);
% off-corridor roadside object
\draw[fill=cdAmberF, draw=cdAmber, line width=0.55pt, rounded corners=0.7pt]
  (3.44,1.46) rectangle (3.72,1.74);

% ---- legend ----------------------------------------------------------
\draw[fill=cdGreenF, draw=cdGreen, line width=0.5pt]
  (0.20,0.38) rectangle (0.36,0.54);
\node[note, anchor=west] at (0.44,0.46) {in-corridor lead vehicle};
\draw[fill=cdAmberF, draw=cdAmber, line width=0.5pt]
  (0.20,0.12) rectangle (0.36,0.28);
\node[note, anchor=west] at (0.44,0.20) {off-corridor roadside object};
\end{scope}


==> figures/fig1/panel_b.tex <==
% =====================================================================
%  Fig. 1, panel (b): the PCR audit. Two measured signals, fused under a
%  physics hard gate. Numbers are the per-category means of Table I.
%  Local frame: (0,0) bottom-left, 6.20 x 4.60 cm.
% =====================================================================
\begin{scope}[shift={(\pBx,\pRowy)}]
\def\W{6.20}\def\H{4.60}
\draw[panel] (0,0) rectangle (\W,\H);

\node[ptitle] at (0.16,\H-0.30) {(b) \pcr: physics-grounded causal audit};
\node[psub]   at (0.16,\H-0.55)
  {contrast what the planner uses with what physics permits};

% ---- helper: labelled value bar (uses \bx as the bar origin) ---------
% #1 y, #2 label, #3 value in [0,1], #4 colour
\def\vbar#1#2#3#4{%
  \node[note, anchor=east] at (\bx-0.06,#1) {#2};
  \draw[cdLine, line width=0.35pt] (\bx,#1-0.052) rectangle (\bx+1.06,#1+0.052);
  \fill[#4] (\bx,#1-0.052) rectangle (\bx+1.06*#3,#1+0.052);
  \node[note, anchor=west, text=#4!70!black] at (\bx+1.12,#1) {#3};}

% =========================== card 1: influence =======================
\draw[card] (0.16,2.02) rectangle (3.08,3.90);
\fill[cdSlate] (0.34,3.70) circle (0.10);
\node[font=\cdtiny, text=white] at (0.34,3.70) {1};
\node[anchor=west, font=\cdtiny\bfseries] at (0.48,3.70)
  {Model influence $\tilde I_i$};
\node[note, anchor=west] at (0.26,3.46) {$r_i=\|a-a_{\setminus i}\|_2$};
\node[note, anchor=west] at (0.26,3.26) {$\tilde I_i=r_i/\max_j r_j$};
{\def\bx{1.22}
 \vbar{2.98}{lead veh.}{0.76}{cdGreen}
 \vbar{2.72}{roadside}{0.84}{cdAmber}}
\node[note, anchor=north west, text width=2.62cm] at (0.26,2.50)
  {high for both, so influence alone cannot separate them};

% =========================== card 2: physics prior ===================
\draw[card] (3.20,2.02) rectangle (6.04,3.90);
\fill[cdBlue] (3.38,3.70) circle (0.10);
\node[font=\cdtiny, text=white] at (3.38,3.70) {2};
\node[anchor=west, font=\cdtiny\bfseries] at (3.52,3.70)
  {Physics prior $\rho_i$};
\node[note, anchor=west] at (3.30,3.46)
  {$\rho_i=c_i\max(\pi_i,\tau_i)\,\omega_{\kappa_i}$};
\node[note, anchor=west] at (3.30,3.26) {corridor overlap, TTC, class};
{\def\bx{4.26}
 \vbar{2.98}{lead veh.}{0.78}{cdGreen}
 \vbar{2.72}{roadside}{0.06}{cdAmber}}
\node[note, anchor=north west, text width=2.54cm] at (3.30,2.50)
  {\textbf{external anchor}: geometry, not data};

% ---- both signals feed the fusion -----------------------------------
\draw[flow] (1.62,2.02) -- (1.62,1.72);
\draw[flow] (4.62,2.02) -- (4.62,1.72);

% =========================== fusion ==================================
\draw[well] (0.16,0.14) rectangle (6.04,1.72);
\node[font=\cdsmall] at (3.10,1.48)
  {$\mathrm{PCR}_i=\tilde I_i\,(1-\rho_i)\,(1+\lambda\sigma_i)$};
\node[chipG] at (3.10,1.20)
  {hard gate\ \ $\rho_i\ge\rho_{\mathrm{hi}}\Rightarrow\mathrm{PCR}_i=0$};
\node[note, text=cdSlate] at (3.10,0.96)
  {a physically plausible query is never flagged};

\node[chipG, anchor=north west, align=left] at (0.30,0.80)
  {\textbf{lead veh.}\ \ $\rho\,0.78\ge\rho_{\mathrm{hi}}$\\[0.8pt]
   gate protects: $\mathrm{PCR}_i=0$};
\node[chipA, anchor=north west, align=left] at (3.20,0.80)
  {\textbf{roadside}\ \ $\tilde I\,0.84$, $\rho\,0.06$\\[0.8pt]
   \textbf{flagged}: $\mathrm{PCR}_i=0.79$};
\end{scope}


==> figures/fig1/panel_c.tex <==
% =====================================================================
%  Fig. 1, panel (c): TCM. Rank queries by PCR, mask above threshold,
%  re-plan. Local frame: (0,0) bottom-left, 5.10 x 4.60 cm.
% =====================================================================
\begin{scope}[shift={(\pCx,\pRowy)}]
\def\W{5.10}\def\H{4.60}
\draw[panel] (0,0) rectangle (\W,\H);

\node[ptitle] at (0.16,\H-0.30) {(c) \tcm: test-time masking};
\node[psub] (csub) at (0.16,\H-0.55)
  {one extra forward pass, no parameter update};
\pic at ([xshift=1.9mm]csub.east) {snow};

% ---- PCR spectrum with the flagging threshold -----------------------
\draw[well] (0.16,2.56) rectangle (\W-0.16,3.90);
\def\gy{2.96}\def\gh{0.80}
\foreach \k/\v in {0/0.92,1/0.79,2/0.34,3/0.24,4/0.17,
                   5/0.12,6/0.08,7/0.05,8/0.03,9/0.01}{
  \pgfmathsetmacro{\bxx}{0.76+\k*0.385}
  \ifnum\k<2
    \fill[cdAmber] (\bxx,\gy) rectangle (\bxx+0.24,\gy+\gh*\v);
    \draw[cdAmber, line width=0.6pt]
      (\bxx+0.05,\gy+\gh*\v+0.08) -- (\bxx+0.19,\gy+\gh*\v+0.20)
      (\bxx+0.05,\gy+\gh*\v+0.20) -- (\bxx+0.19,\gy+\gh*\v+0.08);
  \else
    \fill[cdSlate!42] (\bxx,\gy) rectangle (\bxx+0.24,\gy+\gh*\v);
  \fi}
\draw[cdSlate, line width=0.4pt] (0.68,\gy) -- (\W-0.44,\gy);
\draw[cdGreen, line width=0.5pt, dash pattern=on 1.6pt off 1.3pt]
  (0.64,\gy+0.5*\gh) -- (\W-0.38,\gy+0.5*\gh);
\node[note, anchor=west, text=cdGreen!62!black]
  at (\W-0.36,\gy+0.5*\gh) {$\theta$};
\node[note, rotate=90, text=cdSlate] at (0.44,\gy+0.30) {$\mathrm{PCR}_i$};
\node[note, anchor=north, text=cdSlate] at (2.60,\gy-0.08)
  {agent queries, ranked};

% ---- the masking operator -------------------------------------------
\node[chipB, font=\cdsmall, inner ysep=2.4pt] (op) at (2.60,2.29)
  {$a^{\dagger}=f_{\setminus F}(Q,e)$,\ \ $F=\{i:\mathrm{PCR}_i>\theta\}$};
\draw[flow] (2.60,2.56) -- (op.north);
\draw[flow] (op.south) -- (2.60,2.02);

% ---- deconfounded outcome -------------------------------------------
\draw[well] (0.16,0.16) rectangle (\W-0.16,2.02);
\def\rb{0.52}\def\rt{1.90}
\fill[cdBlueF] (1.05,\rb) -- (3.45,\rb) -- (2.60,\rt) -- (1.90,\rt) -- cycle;
\draw[cdBlue!38, line width=0.4pt]
  (1.05,\rb) -- (1.90,\rt)  (3.45,\rb) -- (2.60,\rt);

\fill[cdInk!88, rounded corners=0.7pt] (1.99,0.58) rectangle (2.51,0.86);
\draw[fill=cdGreenF, draw=cdGreen, line width=0.55pt, rounded corners=0.7pt]
  (2.07,1.43) rectangle (2.43,1.62);

% flagged object, suppressed at inference
\draw[fill=cdAmberF!55, draw=cdAmber!50, line width=0.5pt,
      rounded corners=0.7pt] (3.62,0.96) rectangle (3.90,1.24);
\draw[cdAmber, line width=0.7pt]
  (3.62,0.96) -- (3.90,1.24)  (3.62,1.24) -- (3.90,0.96);
\node[note, anchor=west, text=cdAmber!70!black] at (3.98,1.10) {masked};

% baseline plan against the deconfounded plan
\foreach \y in {0.96,1.08}{\fill[cdSlate!60] (2.05,\y) circle (0.036);}
\foreach \y in {0.96,1.08,1.20,1.32}{\fill[cdBlue] (2.45,\y) circle (0.038);}
\node[note, anchor=east, text=cdSlate] at (1.97,1.02) {$a$};
\node[note, anchor=west, text=cdBlue!80!black] at (2.53,1.28)
  {$a^{\dagger}$};
\node[note, anchor=south, text=cdSlate] at (2.55,0.22)
  {maneuver preserved, flagged reliance removed};
\end{scope}


==> figures/fig1/panel_d.tex <==
% =====================================================================
%  Fig. 1, panel (d): the counterfactual benchmark, drawn as a base plate
%  under the pipeline because it probes the same frozen planner.
%  Local frame: (0,0) bottom-left, \Wtot x 1.50 cm.
% =====================================================================
\begin{scope}
\def\H{1.50}
\draw[panel] (0,0) rectangle (\Wtot,\H);

\node[anchor=north west, font=\footnotesize\bfseries, align=left,
      inner sep=0pt] at (0.16,\H-0.20)
  {(d) Counterfactual\\[1.5pt]robustness benchmark};
\node[note, anchor=north west, text width=2.62cm] at (0.16,\H-0.82)
  {query-level probes, applied before and after \tcm};

\draw[hair] (2.98,0.16) -- (2.98,\H-0.16);
\draw[hair] (7.68,0.16) -- (7.68,\H-0.16);
\draw[hair] (12.38,0.16) -- (12.38,\H-0.16);

% #1 x origin, #2 probe, #3 expected behaviour, #4 metric, #5 colour
\def\probeitem#1#2#3#4#5{%
  \node[anchor=west, font=\cdsmall] at (#1,\H-0.50) {#2};
  \node[note, anchor=north west, text width=3.05cm] at (#1,\H-0.72) {#3};
  \node[chip, draw=#5, fill=#5!8, text=#5!72!black, anchor=east,
        font=\cdsmall, inner ysep=2.6pt] at (#1+4.28,\H-0.72) {#4};}

\probeitem{3.16}{perturb a \textbf{spurious} query}
  {$\rho\!\approx\!0$, so the plan must not move}{CSI $\uparrow$}{cdAmber}
\probeitem{7.86}{perturb a \textbf{causal} query}
  {a lead vehicle brakes, so the plan must respond}{CRI $\uparrow$}{cdGreen}
\probeitem{12.56}{apply a \textbf{distribution shift}}
  {day to night, so the plan must stay consistent}{CCS $\uparrow$}{cdBlue}
\end{scope}

